Efficient Nonlinear RX Anomaly Detectors

Current anomaly detection algorithms are typically challenged by either accuracy or efficiency. More accurate nonlinear detectors are typically slow and not scalable. In this letter, we propose two families of techniques to improve the efficiency of the standard kernel Reed-Xiaoli (RX) method for anomaly detection by approximating the kernel function with either {\em data-independent} random Fourier features or {\em data-dependent} basis with the Nystr\"om approach. We compare all methods for both real multi- and hyperspectral images. We show that the proposed efficient methods have a lower computational cost and they perform similar (or outperform) the standard kernel RX algorithm thanks to their implicit regularization effect. Last but not least, the Nystr\"om approach has an improved power of detection.

==> keywords.tex <==
\begin{IEEEkeywords}
Anomaly detection, hyperspectral, RX detector, nonlinear methods, kernel methods, randomization, randomized feature maps, low-rank approximation, Nystr\"om method
\end{IEEEkeywords}


==> methods_Nystrom_OLD.tex <==
The Nystr\"om method selects a subset of samples to construct a low-rank approximation of the kernel matrix~\cite{Nystrom}.
In the Nystr\"om method the kernel function $K$ is approximated as follows
\begin{equation}
K_{\text{Nystr\"om}}(\x_i, \x_j) = K_{\x_i:r}^\top{\hat\K}^{-1} K_{r:\x_j}^\top,
\end{equation} 
where $\hat{\K}\in\Real^{r\times r}$ stands for the kernel matrix containing data similarities between the points in $\hat\X$.
\iffalse
    % details of the derivation of low-rank in Hilbert space
    Accordingly, $k(\x_\ast,\x_j)$ is defined as
    \begin{equation}
    k(\x_\ast, x_j) \approx k_{\text{Nystr\"om}}(\x_\ast, x_j) = k(\x_\ast, \hat\X)^\top {\hat\K}^{-1} k(\hat\X, x_j)
    \end{equation} 
    where $k(x_\ast, \hat\X) \in \Real^{r}$ contains similarities between $\x_\ast$ and $\hat\X$ and $k(\hat\X, x_j) \in \Real^{r}$ contains similarities between $\hat\X$ and $\x_j$, both using kernel function $k$. 
    
    At last, ${\bf k}_\ast = [k(\x_\ast,\x_1),\ldots, k(\x_\ast,\x_n)]^\top\in\Real^{n}$ can be defined as:
    \begin{equation}
     {\bf k}_\ast \approx [k_{\text{Nystr\"om}}(\x_\ast,\x_1),\ldots, k_{\text{Nystr\"om}}(\x_\ast,\x_n)]^\top
    \end{equation} 
    which is
    \begin{equation}
     {\bf k}_\ast \approx [k(\x_\ast, \hat\X)^\top {\hat\X}^{-1} k(\hat\X, x_1), \ldots, k(\x_\ast, \hat\X)^\top {\hat\X}^{-1} k(\hat\X, x_n)]^\top
    \end{equation} 
    
    Let's define $k(x_\ast, \hat\X)$ as ${\bf k}_{\ast:r}$ as a vector with size of $r \times 1$ and $\acute{\K}\in\Real^{r \times n}$ as a matrix which contains similarities between the points in $\hat\X$ and all points in $\X$.
\fi
Then, after some algebraic manipulations, ${\bf k}_\ast$ can be expressed as:
\begin{equation}
 \label{eq:kstar_approximation}
 {\bf k}_\ast \approx  {\R}^\top {\hat\K}^{-1} {\bf k}_{\ast:r}
\end{equation} 
where ${\R}\in\Real^{r \times n}$ is a matrix which contains similarities between the points in $\hat\X$ and the points in $\X$. 

Using the above definition given in Equation~\eqref{eq:kstar_approximation}, Nystr\"om method defines the kernel matrix $\K$ as:
\begin{equation}
 \label{eq:K_approximation}
 \K \approx {\R}^\top {\hat\K}^{-1} {\R}
\end{equation} 
Then, by assigning the Equation~\eqref{eq:kstar_approximation} and \eqref{eq:K_approximation} into the Equation~\eqref{eq:krx}, we can define the low-rank approximation of KRX as below:
\iffalse
    % intermediary step between above and below equations 
    \begin{equation}
    D_{NRX}(\x_\ast) = {\bf k}_\ast^\top ({\R}^\top {\hat\K}^{-1} {\R} {\R}^\top {\hat\K}^{-1} {\R})^{-1} {\bf k}_\ast,
    \end{equation}
    or equivalently
\fi
\begin{equation}
\label{eq:nrx2}
D_{NRX}(\x_\ast) = 
{\bf k}_{\ast:r}^\top {\hat\K}^{-1} {\R}
({\R}^\top \M {\R})^{-1} 
{\R}^\top {\hat\K}^{-1} {\bf k}_{\ast:r},
\end{equation} 
where $\M = {\hat\K}^{-1} {\R} {\R}^\top {\hat\K}^{-1}$ while $\M \in\Real^{r \times r}$. 
Since, $\R$ is not a square matrix, one can use the pseudoinverse instead:
\begin{equation}
\label{eq:nrx3}
D_{NRX}(\x_\ast) = 
{\bf k}_{\ast:r}^\top {\hat\K}^{-1} {\R}
({\R}^{\dagger} {\M}^{-1}  {\R}^{{\dagger}^{\top}})
{\R}^\top {\hat\K}^{-1} {\bf k}_{\ast:r},
\end{equation}
where ${\R}^{\dagger} \in\Real^{n \times r}$ by definition.
Finally, NRX is defined as 
\begin{equation}
\label{eq:nrx}
D_{NRX}(\x_\ast) = {\bf k}_{\ast:r}^\top ({\V}^{\top} {\M}^{-1} {\V}) {\bf k}_{\ast:r},
\end{equation} 
where $\V = {\R}^{{\dagger}^{\top}} {\R}^{\top} {\hat\K}^{-1} \in\Real^{r \times r}$. 
Note that NRX is much more efficient comparing to KRX since both $\V$ and $\M$ are matrices with size $r \times r$ and $r \ll n$.
\textcolor{blue}{The Nyström approach is more generic than Fourier features approaches in the sense that the later are limited to shift-invariant kernel functions (e.g. RBF). 
This feature makes the Nyström approach more flexible and able to be implemented with any positive semidefinite (PSD) kernel function.}

==> methods_RFF_RX.tex <==
Given $n$ data points (pixels), the kernel matrix ${\bf K} \in\Real^{n\times n}$ can be approximated with the explicitly mapped data, ${\bf Z}=[{\bf z}_1\cdots{\bf z}_n]^\top\in\Real^{n\times D}$, and will be denoted as $\hat{\bf K}\approx{\bf Z}{\bf Z}^\top.$ 
However, we do not use such approximation in Eq.~\eqref{eq:krx} which would lead to a mere approximation with extra computational cost. 
Instead, we run the linear RX in Eq.~\eqref{eq:rx} with explicitly mapped points onto random Fourier features, which reduces to
\begin{equation}
D_{RRX} = \Re{\left(\z_\ast^\top(\Z^\top\Z)^{-1}\z_\ast\right)},
\end{equation}
where $\z_\ast = \z(\x_\ast)$, and $\Re$ is the real part function $\Re{\left(a+\imag b\right)}=a$. 
This leads to a nonlinear randomized RX (RRX) that approximates the KRX in expectation. 
Essentially, we map the original data $\x_i$ into a nonlinear space through the explicit mapping $\z(\x_i)$ to a $D$-dimensional space (instead of the potentially infinite feature space with $\boldsymbol{\phi}(\x_i)$), and then use the linear RX formula.
This allows to control the space and time complexity explicitly through $D$, as one has to store matrices of $n\times D$ and invert matrices of size $D\times D$ only.
Typically, parameter $D$ satisfies $D\ll n$ in practical applications, which turns to be a beneficial regularization effect in the solution.

